Encoding Range Minimum Queries

We consider the problem of encoding range minimum queries (RMQs): given an array A[1..n] of distinct totally ordered values, to pre-process A and create a data structure that can answer the query RMQ(i,j), which returns the index containing the smallest element in A[i..j], without access to the array A at query time. We give a data structure whose space usage is 2n + o(n) bits, which is asymptotically optimal for worst-case data, and answers RMQs in O(1) worst-case time. This matches the previous result of Fischer and Heun [SICOMP, 2011], but is obtained in a more natural way. Furthermore, our result can encode the RMQs of a random array A in 1.919n + o(n) bits in expectation, which is not known to hold for Fischer and Heun's result. We then generalize our result to the encoding range top-2 query (RT2Q) problem, which is like the encoding RMQ problem except that the query RT2Q(i,j) returns the indices of both the smallest and second-smallest elements of A[i..j]. We introduce a data structure using 3.272n+o(n) bits that answers RT2Qs in constant time, and also give lower bounds on the effective entropy} of RT2Q.

==> notation.tex <==
\begin{tabular}{cl}
  \\
  Notation & Description \\
  \hline
  $A$ &  input array \\
  $n$ & the size of $A$\\ 
  $x,y$ & nodes in trees \\
  $i,j,k$ & indexes in $A$ \\
  $h$ & index in $A$ which is the first minimum in a range \\
  $u,v$ & node in the Cartesian tree \\
  \lspine{\cdot}, \rspine{\cdot} \qquad & left/right spine \\
  \lspinebit{\cdot}, \rspinebit{\cdot} & bit sequence of left/right spine \\ 
  $L,R$ & bit vectors for left/right spines \\
  $T_A$ & Cartesian tree\\
  $OT1(T_A)$ & ordinal tree of $T_A$ \\
  $r$ & rank of a node on spine \\
  $B$ & bit vector \\
\end{tabular}


